Code Researcher: Deep Research Agent for Large Systems Code and Commit History

Large Language Model (LLM)-based coding agents have shown promising results on coding benchmarks, but their effectiveness on systems code remains underexplored. Due to the size and complexities of systems code, making changes to a systems codebase requires researching about many pieces of context, derived from the large codebase and its massive commit history, before making changes. Inspired by the recent progress on deep research agents, we design the first deep research agent for code, called Code Researcher, and apply it to the problem of generating patches to mitigate crashes reported in systems code. Code Researcher performs multi-step reasoning about semantics, patterns, and commit history of code to retrieve all relevant context from the codebase and its commit history. We evaluate Code Researcher on kBenchSyz, a benchmark of Linux kernel crashes, and show that it significantly outperforms strong baselines, achieving a crash-resolution rate (CRR) of 48%, compared to 31.5% by SWE-agent and 31% by Agentless, using OpenAI's GPT-4o model. Scaling up sampling budget to 10 trajectories increases Code Researcher's CRR to 54%. Code Researcher is also robust to model choices, reaching 67% with the newer Gemini 2.5-Flash model. Through another experiment on an open-source multimedia software, we show the generalizability of Code Researcher and also conduct ablations. Our experiments highlight the importance of global context gathering and multi-faceted reasoning for large codebases.

==> sections/reproducibility.tex <==
\section*{Reproducibility statement}

We provide all the necessary information to reproduce our results.
In Section~\ref{sec:experiments}, we include details about our benchmarks and the implementation hyperparameters for \cresearcher{} and all the other baselines.
In Appendix~\ref{app:details}, we give details about our subset of the \kbenchsyz{} benchmark, and provide information about the crash reproduction setup, the unit test setup, compute resources, prompts, and the implementation of the SWE-agent and Agentless baselines.
In Appendix~\ref{app:ffmpeg}, we give the complete steps to recreate our dataset for \ffmpeg{} and reproduce our results.
We also present implementation details for \cresearcher{} in Appendix~\ref{app:design}.
Finally, we submit a supplementary zip file containing (a) the full code of our implementation, (b) prompts and config files used for \cresearcher{} and the SWE-agent and Agentless baselines, (c) both the datasets we used, (d) the patches produced by \cresearcher{} and each baseline, and (e) a \texttt{README} that explains how to reproduce our results.
